Conclave: secure multi-party computation on big data (extended TR)

Secure Multi-Party Computation (MPC) allows mutually distrusting parties to run joint computations without revealing private data. Current MPC algorithms scale poorly with data size, which makes MPC on "big data" prohibitively slow and inhibits its practical use. Many relational analytics queries can maintain MPC's end-to-end security guarantee without using cryptographic MPC techniques for all operations. Conclave is a query compiler that accelerates such queries by transforming them into a combination of data-parallel, local cleartext processing and small MPC steps. When parties trust others with specific subsets of the data, Conclave applies new hybrid MPC-cleartext protocols to run additional steps outside of MPC and improve scalability further. Our Conclave prototype generates code for cleartext processing in Python and Spark, and for secure MPC using the Sharemind and Obliv-C frameworks. Conclave scales to data sets between three and six orders of magnitude larger than state-of-the-art MPC frameworks support on their own. Thanks to its hybrid protocols, Conclave also substantially outperforms SMCQL, the most similar existing system.

==> algorithms.tex <==
\begin{algorithm}[]
    \label{alg:join-single}
    \KwData{Secret-shared relation \textit{left}, secret-shared relation \textit{right}, policy $P$ that permits party $P_{1}$ to learn the key-column data of $left$ and $right$. $P_{\textit{all}}$ is the set of all parties.}
    \KwResult{Result of join of \textit{left} and \textit{right} secret-shared across $P_{\textit{all}}$}
    \Begin(Performed by $P_{\textit{all}}$){
        $\text{flte} \gets \text{shuffle(left)}$\;
        $\text{hrtig} \gets \text{shuffle(right)}$\;

        $\text{left}_{\text{keys}} \gets \text{store}(\text{keys}(\text{flte}), \{P_{1}\})$\;
        $\text{right}_{\text{keys}} \gets \text{store}(\text{keys}(\text{hrtig}), \{P_{1}\})$\;
    }

    \Begin(Performed by $P_{1}$){
        $\text{indices}_{P_{1}} \gets \text{indexJoin}(\text{left}_{\text{keys}}, \text{right}_{\text{keys}})$\;
        $\text{indices} \gets \text{store}(\text{indices}_{P_{1}}, \{P_{1}\}, ..., \{P_{n}\})$\;
    }

    \Begin(Performed by $P_{\textit{all}}$){
        $\text{result} \gets \text{joinFromIndices}(\text{flte}, \text{hrtig}, \text{indices})$
    }
    \KwRet result\;

    \tcc{Below functions are self-explanatory}
    \SetKwProg{Fn}{Function}{ is}{end}
    \Fn{indexJoin(left, right)}{
        indices $\gets \{\}$\;
        \For{$i_{l}$, $k_{l}$, $v_{l}$ $\in$ $\textit{left}$}{
            \For{$i_{r}$, $k_{r}$, $v_{r}$ $\in$ $\textit{right}$}{
                \If{$k_{l} = k_{r}$}{
                    add ($i_{l}$, $i_{r}$) to indices
                }
            }
        }
        \KwRet indices\;
    }
    \Fn{joinFromindices(left, right, indices)}{
        result $\gets \{\}$\;
        \For{$i_{l}$, $i_{r}$ $\in$ $\textit{indices}$}{
            $k_{l}, v_{l} \gets \text{tuple at index } i_{l} \text{ in left}$\;
            $k_{r}, v_{r} \gets \text{tuple at index } i_{r} \text{ in right}$\;
            add ($k_{l}$, $v_{l}$, $v_{r}$) to result
        }
        \KwRet result\;
    }
    \caption{Join with all key-column data revealed to single party.}
\end{algorithm}

\begin{algorithm}[]
    \KwData{Relations $\textit{left}_{1}$, ..., $\textit{left}_{m}$ each stored in the clear by $P_{1}$, ..., $P_{m}$ respectively. Secret-shared relation $\textit{right}$. Policy $P$ that allows all parties in $P_{left} = \{P_{1}, ..., P_{m}\}$ to learn the keys of \textit{right}. $P_{\textit{all}} = P_{1}, ..., P_{n}$ is the set of all participating parties. $\textit{left} = \text{concat}(\textit{left}_{1}, ..., \textit{left}_{m})$.}
    \KwResult{Result of join of \textit{left} and \textit{right} secret-shared across $P_{\textit{all}}$.}
    \Begin(Performed by each $P_{i} \in P_{\textit{left}}$){
        $\textit{left}_{i} \gets \text{project}(\textit{left}_{i}, (k, v) \mapsto (k, v, P_{i}))$\;
        $\textit{left}_{i} \gets \text{store}(\textit{left}_{i}, P_{\textit{all}})$
    }
    \Begin(Performed by $P_{\textit{all}}$){
        $\textit{flte} \gets \text{shuffle}(\text{concat}(\textit{left}_{1}, ..., \textit{left}_{m}))$\;
        $\textit{hrtig} \gets \text{shuffle}(\textit{right})$\;
        $\textit{flte} \gets \text{project}(\textit{flte}, (k, v, p) \mapsto (k, p))$\;
        \For{$P_{i} \in P_{\textit{left}}$}{
            $\textit{left}_{k, i} \gets \text{store}(\text{condmask}(\textit{flte}, P_{i}), P_{i})$\;
        }
        $\textit{right}_{\textit{keys}} \gets \text{store}(\text{keys}(\textit{hrtig}), \{P_{1}\}, ..., \{P_{m}\})$\;
    }
    \Begin(Performed by each $P_{i} \in P_{\textit{left}}$){
        $\textit{mine} \gets \text{removeMasked}(\textit{left}_{k, i})$\;
        $\textit{indices}_{i} \gets \text{indexJoin}(\textit{mine}, \textit{right}_{\textit{keys}})$\;
        $\textit{indices}_{i} \gets \text{store}(\textit{indices}_{i}, P_{all})$\;
    }
    \Begin(Performed by $P_{\textit{all}}$){
        $\textit{indices}_{\textit{all}} \gets \text{shuffle}(\text{concat}(\textit{indices}_{1}, ..., \textit{indices}_{m}))$\;
        $\textit{indices}_{\textit{all}} \gets \text{store}(\textit{indices}_{\textit{all}}, \{P_{1}\}, ..., \{P_{n}\})$\;
        $\textit{result} \gets \text{joinFromIndices}(\textit{flte}, \textit{hrtig}, \textit{indices}_{\textit{all}})$\;
    }
    \KwRet result\;
    \SetKwProg{Fn}{Function}{ is}{end}
    \Fn{condmask(rel, P)}{
        $\textit{result} \gets \{\}$\;
        \For{($e_{1}$, ..., $e_{s}$, $P^{\prime}$) $\in$ $\textit{rel}$}{
            $\textit{comp} \gets (P = P^{\prime})$\;
            $\textit{tuple} \gets (\textit{comp}, \textit{comp} * e_{1}, ..., \textit{comp} * e_{s})$\;
            add \textit{tuple} to \textit{result}
        }
        \KwRet \textit{result}\;
    }
    \caption{One-side public key join.}
\end{algorithm}



==> discussion.tex <==
\section{Discussion}
\label{s:discussion}

\todo{Combining MPC paradigms and systems automatically}

\todo{Combine multiple smaller MPCs into a large one}

